Self-supervised language learning from raw audio: Lessons from the Zero Resource Speech Challenge

Recent progress in self-supervised or unsupervised machine learning has opened the possibility of building a full speech processing system from raw audio without using any textual representations or expert labels such as phonemes, dictionaries or parse trees. The contribution of the Zero Resource Speech Challenge series since 2015 has been to break down this long-term objective into four well-defined tasks -- Acoustic Unit Discovery, Spoken Term Discovery, Discrete Resynthesis, and Spoken Language Modeling -- and introduce associated metrics and benchmarks enabling model comparison and cumulative progress. We present an overview of the six editions of this challenge series since 2015, discuss the lessons learned, and outline the areas which need more work or give puzzling results.

==> v2/reviews.tex <==

====
For regular papers, the revised manuscript may not exceed 16 double-column pages (10 point font), including title; names of authors and their complete contact information; abstract; text; all images, figures and tables, appendices and proofs; and all references.
===

Reviewer: 1



Some important discussions are also left to the supplementary material, although they would deserve to be in the main text or at least as an appendix.
- provide more details in Table II. ... some of this information may be already in Table S1, but since this table is not mentioned in the text, nor described, I am not sure about it.
- Many expressions and notations are not defined or defined only in the supplementary material. First, I think that the supplementary material is more of an appendix, and should be included in the main paper. For example, the readers cannot see what the different systems are without looking at Table S2.
- Ideally, the definition of the metrics used in the discussion of the main part of the paper should also be moved to the main part, unless they are relatively obvious to most readers. 





=======


Reviewer: 1



Some important discussions are also left to the supplementary material, although they would deserve to be in the main text or at least as an appendix.

Finally, many of the systems discussed in the paper are not shown in the figures presenting the results. This makes it hard to appreciate how well those systems perform. 

1.	The philosophy behind each task is clearly explained. However, I had trouble understanding the details. For example, a key part to understanding well each task would be Table I. However, Table I contains much information, which is not clearly explained in the text. This table is only briefly mentioned at the end of the introduction. The authors should guide the reader better through the information in the table, probably also mentioning concrete examples of test utterances and the results expected instead of the relatively abstract examples provided in Table I.

Also, please clearly define all notations. As an example, A and B are not defined in the table, nor are s_1, s_i, or U. It may also be helpful to provide some demo samples for each task, providing a test sample and an example of a result.

2.	Could you also provide more details in Table II. For example, what is the ABX test set? Does it consist of utterances or single words, or else? Is it read-speech or spontaneous speech? How many speakers, how much data is it? What is the length of utterances etc.? It would be better to summarize such information so that the reader can better grasp the tasks without having to read the challenge webpage. The same hold for the other tasks. some of this information may be already in Table S1, but since this table is not mentioned in the text, nor described, I am not sure about it.

3.	Many expressions and notations are not defined or defined only in the supplementary material. First, I think that the supplementary material is more of an appendix, and should be included in the main paper. For example, the readers cannot see what the different systems are without looking at Table S2.

Ideally, the definition of the metrics used in the discussion of the main part of the paper should also be moved to the main part, unless they are relatively obvious to most readers. 

4.	Please define clearly all expressions and notations the first time they appear in the text. Some examples are the notations used in Table I, but also some abbreviations such as DPGMM, CPC, etc. are not defined.

Finally, the terminology is sometimes unclear. You mention gold transcription for some tasks, but you do not explain what they are and how they are obtained.

For task 3, what does the “surprise test language” mean? Is it that the training set for Indonesian was provided at the same time as the test set, with limited time for development? Did it require to use of exactly the same system as for English? How was this task still a surprise for the 2020 edition of the challenge? This kind of information may be well known to the challenge participants, but unclear to other readers. 

5.	Many of the systems described in the text are not shown in the figures presenting the results. It is thus unclear how they actually perform.

6.	The paper would be much more informative if Table S2 would be augmented with a brief description of the key components of each system and probably some scores. Or else linking the results with the key technical components for each task as done in Fig. 2.



Reviewer: 2



However, I have several concerns that should be addressed before publication. Specifically, while the authors try to lightly-revisit ALL aspects of ZRCs and cover many systems and results as much as possible (and I can totally understand why the authors would like to do so), it makes the paper rather superficial and makes a take-home-message(s) unclear (if there are any).

The current description may be sufficient for those already familiar with ZRCs, but it is not sufficient for naïve readers.

Overall, I feel that naive readers need a more detailed explanation of the task, evaluation metrics (which are not indeed trivial as mentioned in the paper), and top-performing systems that worked well for each task.

Since such information is indeed what general readers are looking for, I would suggest the authors adjust the “balance” of the paper and provide more detailed information on the following items: (1) each task and its evaluation metrics in the body text (not in the supplemental materials section) hopefully with more equations, and (2) systems that are worth being mentioned more carefully with some accompanying figures/equations, so that people who did not involve in the challenges can understand the critical progress made in the challenges based on well-thought-out metrics.


- Concerning evaluation metrics:
As the authors mentioned in introduction, “The ZRC series has been designed to address two interlocking research problems: the task problem and the evaluation problem”, the evaluation metrics are essential parts of the challenge. On the other hand, the current description of evaluation metrics in the body text is too brief and ambiguous. Consider putting back the description of the evaluation metrics in the supplemental materials section to the text body and merging explanations.
 
- Concerning technical details of submitted systems:
The description of the submitted systems is also too brief. If readers are not already familiar with them before reading the paper, it may be hard for them to follow the paper. Add some more details such as block diagrams or equations, especially to the ones that performed well or provided important progress (For example, it is not easy to imagine what is DPGMM from the current description precisely).

Accordingly, the authors may have to shorten the description of the other less effective or less important methods or completely omit them to meet the page restriction. You can do so by clearly mentioning something like “In this paper, we focus on …. There are some other interesting ideas explored in the ZRC series but not mentioned in the paper. Although they have not reached the top of the leaderboard, they may still have much to contribute, perhaps in combination with other approaches.”

- Concerning baseline systems: 
Most of the time, it is not very clear what is the baseline system in each task (Especially task 4). The author should add a little more explanation about baseline systems too.

- Concerning future challenges and future tasks:
From the reviewer’s point of view, it is not essential to discuss future challenges in this paper in detail. The current description of the future challenge looks more like an advertisement rather than content in a technical journal paper. Just talking about future challenges and new tasks, e.g., Section III-B, C, D, without providing some facts (such as the baseline system and its performance) is not convincing. It would be best if the authors drastically shortened the description of a future challenge (or entirely omitted them), and instead added more critical “facts” to the paper, such as an explanation of the submitted systems, results analysis, and evaluation metrics used in each task, i.e., something we already have.


- In Fig. 5, it is not always clear which data point corresponds to which submission. Make it clear by, e.g., drawing a line between the submission name and a data point.

- It is unclear to me exactly what message the authors would like to convey for Task 4. While they say, in the last paragraph of Section II-D, “Task 4 is clearly in its very early stages,” implying that the overall performance level achieved for Task4 is not satisfactory, in the first paragraph of Section III, they say, “Spoken Language Modeling (T4) got surprisingly promising results”. Sort out these explanations that seemingly contradict each other. 


Reviewer: 3


In my opinion this is an excellent literature review of the type that very much lacking in our field.  The review goes beyond simple summary of prior work and presents a novel, opinionated analysis that gives a reader a sense of what has actually been learned from the 100+ papers in the ZRC.

In particular, I found the distinction between the "task" and "evaluation" problems to be compelling and useful as the different sub-tasks in the challenge were analyzed.  I was also grateful for summaries of the tradeoffs discovered in the individual problems, which is a critical piece of practical knowledge that in the absence of this paper would be left by the reader to infer from a large literature.  

You briefly mention at several points the apparent usefulness of contrastive approaches like CPC.  I would ask you to consider, as another "lesson learned", what seems to be the superiority of techniques that do not model the entirety of the data distribution (as in an autoencoder), and to think about why that is the case.  There is a considerable literature on this topic which is only partially referenced here.  In particular, WavLM should be cited, especially in the discussion of how different audio representations could be necessary for different downstream tasks.

=================================
=================================

ALL REVIEWS:


Reviewer Comments:

Reviewer: 1

Recommendation: RQ-Review Again after Major Changes

Comments:
The paper presents an overview of the zero resource speech challenge activity. It introduces four zero resource tasks and presents the key results of these tasks. Besides, it also discusses overall findings and future directions for the challenge series.
I was not familiar with the challenge activities, but I found the topic and motivation for the challenge very interesting. Also summarizing the outcome of this activity is definitely very informative for the community. I appreciate the great effort the authors have performed to achieve this. 
However, I feel that the paper lacks in terms of clarity in the presentation. The paper seems to assume that the reader is already well familiar with the challenge activity, and many of the tasks, concepts and evaluation metrics are not clearly presented. Some important discussions are also left to the supplementary material, although they would deserve to be in the main text or at least as an appendix. Finally, many of the systems discussed in the paper are not shown in the figures presenting the results. This makes it hard to appreciate how well those systems perform. 
I believe that improving the presentation could make the paper more accessible to a large audience.

Below are some detailed comments.

1.	The philosophy behind each task is clearly explained. However, I had trouble understanding the details. For example, a key part to understanding well each task would be Table I. However, Table I contains much information, which is not clearly explained in the text. This table is only briefly mentioned at the end of the introduction. The authors should guide the reader better through the information in the table, probably also mentioning concrete examples of test utterances and the results expected instead of the relatively abstract examples provided in Table I. Also, please clearly define all notations. As an example, A and B are not defined in the table, nor are s_1, s_i, or U. It may also be helpful to provide some demo samples for each task, providing a test sample and an example of a result.

2.	Could you also provide more details in Table II. For example, what is the ABX test set? Does it consist of utterances or single words, or else? Is it read-speech or spontaneous speech? How many speakers, how much data is it? What is the length of utterances etc.? It would be better to summarize such information so that the reader can better grasp the tasks without having to read the challenge webpage. The same hold for the other tasks. some of this information may be already in Table S1, but since this table is not mentioned in the text, nor described, I am not sure about it.

3.	Many expressions and notations are not defined or defined only in the supplementary material. First, I think that the supplementary material is more of an appendix, and should be included in the main paper. For example, the readers cannot see what the different systems are without looking at Table S2. Ideally, the definition of the metrics used in the discussion of the main part of the paper should also be moved to the main part, unless they are relatively obvious to most readers. 

4.	Please define clearly all expressions and notations the first time they appear in the text. Some examples are the notations used in Table I, but also some abbreviations such as DPGMM, CPC, etc. are not defined. Finally, the terminology is sometimes unclear. You mention gold transcription for some tasks, but you do not explain what they are and how they are obtained. For task 3, what does the “surprise test language” mean? Is it that the training set for Indonesian was provided at the same time as the test set, with limited time for development? Did it require to use of exactly the same system as for English? How was this task still a surprise for the 2020 edition of the challenge? This kind of information may be well known to the challenge participants, but unclear to other readers. 

5.	Many of the systems described in the text are not shown in the figures presenting the results. It is thus unclear how they actually perform.

6.	The paper would be much more informative if Table S2 would be augmented with a brief description of the key components of each system and probably some scores. Or else linking the results with the key technical components for each task as done in Fig. 2.


Additional Questions:
1. Is the topic appropriate for publication in these transactions?: Adequate Match

1. Is the paper technically sound?: Yes

2. How would you rate the technical novelty of the paper?: Novel Enough for Publication

Explain: The paper is an overview paper of the challenge activity. The novelty resides in presenting a summary of the activity, including the major trends and results as well as presenting the remaining challenges.

3. Is the contribution significant?: Significant

4. Is the coverage of the topic sufficiently comprehensive and balanced?: Important Information is missing or superficially treated

5. Rate the Bibliography: Satisfactory

1. How would you rate the overall organization of the paper?: Could be improved

2. Are the title and abstract satisfactory?: Yes

3. Is the length of the paper appropriate? If not, recommend what should be added or eliminated.: Yes

null: 

4. Are symbols, terms, and concepts adequately defined?: No

5. How do you rate the English usage?: Satisfactory


Reviewer: 2

Recommendation: RQ-Review Again after Major Changes

Comments:
This paper summarizes the tasks and results of the six editions of the Zero Resource Speech Challenge (ZRC) series since 2015. It first presents the motivation of the challenge, and shows how each task in the challenge is related to each component of a traditional pipeline used in, e.g., speech-to-speech translation or speech assistants. Then, it revisits each task by briefly introducing its evaluation metrics, various systems submitted to the task, their results, and analysis. The paper is interesting, and it feels like many people in the related research field would appreciate the authors’ effort to put together all this information into one paper.

However, I have several concerns that should be addressed before publication. Specifically, while the authors try to lightly-revisit ALL aspects of ZRCs and cover many systems and results as much as possible (and I can totally understand why the authors would like to do so), it makes the paper rather superficial and makes a take-home-message(s) unclear (if there are any). The current description may be sufficient for those already familiar with ZRCs, but it is not sufficient for naïve readers. Overall, I feel that naive readers need a more detailed explanation of the task, evaluation metrics (which are not indeed trivial as mentioned in the paper), and top-performing systems that worked well for each task. Since such information is indeed what general readers are looking for, I would suggest the authors adjust the “balance” of the paper and provide more detailed information on the following items: (1) each task and its evaluation metrics in the body text (not in the supplemental materials section) hopefully with more equations, and (2) systems that are worth being mentioned more carefully with some accompanying figures/equations, so that people who did not involve in the challenges can understand the critical progress made in the challenges based on well-thought-out metrics.

See the following comments for more details.

- Concerning evaluation metrics:
As the authors mentioned in introduction, “The ZRC series has been designed to address two interlocking research problems: the task problem and the evaluation problem”, the evaluation metrics are essential parts of the challenge. On the other hand, the current description of evaluation metrics in the body text is too brief and ambiguous. Consider putting back the description of the evaluation metrics in the supplemental materials section to the text body and merging explanations.
 
- Concerning technical details of submitted systems:
The description of the submitted systems is also too brief. If readers are not already familiar with them before reading the paper, it may be hard for them to follow the paper. Add some more details such as block diagrams or equations, especially to the ones that performed well or provided important progress (For example, it is not easy to imagine what is DPGMM from the current description precisely). 
Accordingly, the authors may have to shorten the description of the other less effective or less important methods or completely omit them to meet the page restriction. You can do so by clearly mentioning something like “In this paper, we focus on …. There are some other interesting ideas explored in the ZRC series but not mentioned in the paper. Although they have not reached the top of the leaderboard, they may still have much to contribute, perhaps in combination with other approaches.”

- Concerning baseline systems: 
Most of the time, it is not very clear what is the baseline system in each task (Especially task 4). The author should add a little more explanation about baseline systems too.

- Concerning future challenges and future tasks:
From the reviewer’s point of view, it is not essential to discuss future challenges in this paper in detail. The current description of the future challenge looks more like an advertisement rather than content in a technical journal paper. Just talking about future challenges and new tasks, e.g., Section III-B, C, D, without providing some facts (such as the baseline system and its performance) is not convincing. It would be best if the authors drastically shortened the description of a future challenge (or entirely omitted them), and instead added more critical “facts” to the paper, such as an explanation of the submitted systems, results analysis, and evaluation metrics used in each task, i.e., something we already have.

The followings are some minor comments.

- In Fig. 5, it is not always clear which data point corresponds to which submission. Make it clear by, e.g., drawing a line between the submission name and a data point.

- It is unclear to me exactly what message the authors would like to convey for Task 4. While they say, in the last paragraph of Section II-D, “Task 4 is clearly in its very early stages,” implying that the overall performance level achieved for Task4 is not satisfactory, in the first paragraph of Section III, they say, “Spoken Language Modeling (T4) got surprisingly promising results”. Sort out these explanations that seemingly contradict each other. 

Additional Questions:
1. Is the topic appropriate for publication in these transactions?: Excellent Match

1. Is the paper technically sound?: Yes

2. How would you rate the technical novelty of the paper?: Novel Enough for Publication

Explain: The summary of outcomes of Zero Resource Challenge has not been done elsewhere. The paper indeed provides some new analysis results and high-level description of the challenge, which should attract people's interest, and can be seen as a scientific novelty.

3. Is the contribution significant?: Significant

4. Is the coverage of the topic sufficiently comprehensive and balanced?: Important Information is missing or superficially treated

5. Rate the Bibliography: Satisfactory

1. How would you rate the overall organization of the paper?: Could be improved

2. Are the title and abstract satisfactory?: Yes

3. Is the length of the paper appropriate? If not, recommend what should be added or eliminated.: No (Explain):

null: See my comments on the future challenge

4. Are symbols, terms, and concepts adequately defined?: Not always

5. How do you rate the English usage?: Satisfactory


Reviewer: 3

Recommendation: A-Publish Unaltered

Comments:
In my opinion this is an excellent literature review of the type that very much lacking in our field.  The review goes beyond simple summary of prior work and presents a novel, opinionated analysis that gives a reader a sense of what has actually been learned from the 100+ papers in the ZRC.

In particular, I found the distinction between the "task" and "evaluation" problems to be compelling and useful as the different sub-tasks in the challenge were analyzed.  I was also grateful for summaries of the tradeoffs discovered in the individual problems, which is a critical piece of practical knowledge that in the absence of this paper would be left by the reader to infer from a large literature.  

You briefly mention at several points the apparent usefulness of contrastive approaches like CPC.  I would ask you to consider, as another "lesson learned", what seems to be the superiority of techniques that do not model the entirety of the data distribution (as in an autoencoder), and to think about why that is the case.  There is a considerable literature on this topic which is only partially referenced here.  In particular, WavLM should be cited, especially in the discussion of how different audio representations could be necessary for different downstream tasks.

Thank you very much for preparing this manuscript.  I hope to see deep, narrowly-scoped reviews such as this become more common in machine learning.  I believe it would be of great benefit to the community.


Additional Questions:
1. Is the topic appropriate for publication in these transactions?: 

1. Is the paper technically sound?: Yes

2. How would you rate the technical novelty of the paper?: Not Novel

Explain: This manuscript offers no new technology - it's technical contributions are limited to novel analysis of existing ideas.  Nevertheless, I will recommend publication.  The manuscript provides a comprehensive review that while not technically novel, is very much needed in an increasingly sprawling literature.

3. Is the contribution significant?: Significant

4. Is the coverage of the topic sufficiently comprehensive and balanced?: Yes

5. Rate the Bibliography: Satisfactory

1. How would you rate the overall organization of the paper?: Satisfactory

2. Are the title and abstract satisfactory?: Yes

3. Is the length of the paper appropriate? If not, recommend what should be added or eliminated.: Yes

null: 

4. Are symbols, terms, and concepts adequately defined?: Yes

5. How do you rate the English usage?: Satisfactory

